On the Universality of Graph Neural Networks on Large Random Graphs

We study the approximation power of Graph Neural Networks (GNNs) on latent position random graphs. In the large graph limit, GNNs are known to converge to certain "continuous" models known as c-GNNs, which directly enables a study of their approximation power on random graph models. In the absence of input node features however, just as GNNs are limited by the Weisfeiler-Lehman isomorphism test, c-GNNs will be severely limited on simple random graph models. For instance, they will fail to distinguish the communities of a well-separated Stochastic Block Model (SBM) with constant degree function. Thus, we consider recently proposed architectures that augment GNNs with unique node identifiers, referred to as Structural GNNs here (SGNNs). We study the convergence of SGNNs to their continuous counterpart (c-SGNNs) in the large random graph limit, under new conditions on the node identifiers. We then show that c-SGNNs are strictly more powerful than c-GNNs in the continuous limit, and prove their universality on several random graph models of interest, including most SBMs and a large class of random geometric graphs. Our results cover both permutation-invariant and permutation-equivariant architectures.

==> app_approx_sphere.tex <==

\section{Attempt for approximation with dot-product kernel, data on the sphere}

\begin{proposition}[Equivariant case]
\label{prop:dotprod-eq}
    Consider $\Xx = \mathbb S^{d-1}$, $W(x,y) = w(x^\top y)$ a dot-product kernel with an invertible, continuous $w$, and $P$ with a density $f$ with respect to the uniform measure on the sphere. Then: cGWNNs are dense??
\end{proposition}
\begin{proof}
We want to show that if for~$y, y' \in \mathbb S^{d-1}$, and for all continuous function~$g$ we have
\begin{equation}
\label{eq:dotprod_eq_assumption}
\int g(w(y^\top x)) dP(x) = \int g(w(y'^\top x)) dP(x),
\end{equation}
then~$y = y'$.

Denote by~$Y_{k,j}$ with~$k \geq 0$ and~$j = 1, \ldots, N(d,k)$ an orthonormal basis of spherical harmonic polynomials in~$L^2(\mathbb S^{d-1}, d\tau)$, where~$\tau$ is the uniform distribution on the sphere. In particular,~$Y_{k,j}$ a homogeneous harmonic polynomial of degree~$k$.
Let
\begin{equation*}
f(x) = \sum_{k \geq 0} f_k(x) = \sum_{k \geq 0} \sum_{j=1}^{N(d,k)} a_{k,j} Y_{k,j}(x)
\end{equation*}
be the spherical harmonic decomposition of the density~$f$ of~$P$ w.r.t.~$\tau$.

Let~$P_k$ denote the Legendre/Gegenbauer polynomial of degree~$k$, which satisfies the addition formula
\begin{equation*}
P_k(x^\top y) = \frac{1}{N(d,k)} \sum_{j=1}^{N(d,k)} Y_{k,j}(x) Y_{k,j}(y).
\end{equation*}
Then, taking~$g = N(d,k) P_k \circ w^{-1}$, note that we have
\begin{align*}
\int g(w(y^\top x)) dP(x) &= N(d,k)\int P_k(y^\top x) f(x) d \tau(x) \\
	&= \sum_j Y_{k,j}(y) \langle f, Y_{k,j} \rangle_{L^2(d\tau)} \\
	&= f_k(y).
\end{align*}
Thus, \eqref{eq:dotprod_eq_assumption} implies $f_k(y) = f_k(y')$ for all~$k$.

Q: if~$d$ (or just assume infinite number for simplicity?) of the~$f_k$ are non-zero, can we conclude that~$y = y'$? Need at least some~$k$ of different parities if we want to identify $y$ exactly.

Is there a magic result from solutions of polynomial equations? Note that~$f_k$, if non-zero, ``oscillates'' at frequency~$k$, so each equation has a discrete set of solutions for~$k > 0$. But, things might depend on which~$Y_{k,j}$s $f_k$ is supported on...?

For $d=2$ (circle), the equations correspond to~$\cos(k(\theta - \theta_k)) = \cos(k(\theta' - \theta_k))$

\end{proof}



\begin{proposition}[Invariant case]
\label{prop:dotprod-inv}
    Consider $\Xx = \mathbb S^{d-1}$, $W(x,y) = w(x^\top y)$ a dot-product kernel with an invertible, continuous $w$.
\end{proposition}
\begin{proof}
We want to show that if for all $g_1, g_2$
\begin{equation*}
\int g_1(\int g_2(w(x^\top y)) dP(x)) dP(y) = \int g_1(\int g_2(w(x^\top y)) dP'(x)) dP'(y)
\end{equation*}
then~$P = P'$.

Assume densities $f, f'$. Taking~$g_2 = N(d,k) P_k \circ w^{-1}$, we have
\begin{equation*}
\int g_2(w(x^\top y)) dP(x) = f_k(y).
\end{equation*}
With~$g_1(x) = x$ we obtain $\|f_k\| = \|f'_k\|$.

But: unclear if we can properly recover information about specific harmonic components at a given frequency~$k$ using the second layer...

\end{proof}

\todonico{we could do only equivariant. A sufficient condition for universality is: $P$ belongs to 
\begin{equation}
    \{ f = \sum_k f_k ~|~ x \to [f_k(x)]_k \text{ is injective} \}
\end{equation}
maybe that's enough?? I'm not sure we could do much more explicit conditions on the $a_{k,j}$. Also, could we exploit the nonnegativity of $f$ ?
}
